Phase-stable self-modulation of an electron-beam in a magnetic wiggler

Electron-beams with a sinusoidal energy modulation have the potential to emit sub-femtosecond x-ray pulses in a free-electron laser. The energy modulation can be generated by overlapping a powerful infrared laser with an electron-beam in a magnetic wiggler. Here we report on a new infrared source for this modulation, coherent radiation from the electron-beam itself. In this self-modulation process, the current spike on the tail of the electron-beam radiates coherently at the resonant wavelength of the wiggler, producing a six-period carrier-envelope-phase (CEP) stable infrared field with gigawatt power. This field creates a few MeV, phase-stable modulation in the electron-beam core. The modulated electron-beam is immediately useful for generating sub-femtosecond x-ray pulses at any machine repetition rate, and the CEP-stable infrared field may find application as an experimental pump or timing diagnostic.

==> old_table_fig6.tex <==
\iffalse
\begin{table}[b]
\caption{\label{table}%
LCLS beam parameters used for each experiment.
}
\begin{ruledtabular}
\begin{tabular}{lllll}
Parameter & Figs.~2, 3 & Fig.~4 & Fig.~5 & Fig.~6\\
\colrule 
           Wiggler gap (mm)     & 8.2 & 8.2 & 8.2, 16, 20 &11.5\\ 
           Wiggler K-value  &  ?     &   & & \\ 
           Wiggler period (cm)  &  32     & 32  & 32& 32\\ 
           Wiggler length (cm) &     180?  & 180   & 180& 180\\ 
           Resonant period ($\mu$m)  & ?      &   & & \\ 
           Beam energy\footnote{Reported values are set-points, actual values vary shot-to-shot.} (MeV)    &   3953      & 3782 & 3782& 3420\\ 
           Beam charge\textsuperscript{a} (pC)    &  200       & 180 & 180 & 140
\end{tabular}
\end{ruledtabular}
\label{paramtable}
\end{table}
\fi
